Improving Biomedical Information Retrieval with Neural Retrievers

Information retrieval (IR) is essential in search engines and dialogue systems as well as natural language processing tasks such as open-domain question answering. IR serve an important function in the biomedical domain, where content and sources of scientific knowledge may evolve rapidly. Although neural retrievers have surpassed traditional IR approaches such as TF-IDF and BM25 in standard open-domain question answering tasks, they are still found lacking in the biomedical domain. In this paper, we seek to improve information retrieval (IR) using neural retrievers (NR) in the biomedical domain, and achieve this goal using a three-pronged approach. First, to tackle the relative lack of data in the biomedical domain, we propose a template-based question generation method that can be leveraged to train neural retriever models. Second, we develop two novel pre-training tasks that are closely aligned to the downstream task of information retrieval. Third, we introduce the ``Poly-DPR'' model which encodes each context into multiple context vectors. Extensive experiments and analysis on the BioASQ challenge suggest that our proposed method leads to large gains over existing neural approaches and beats BM25 in the small-corpus setting. We show that BM25 and our method can complement each other, and a simple hybrid model leads to further gains in the large corpus setting.

==> error_analysis.tex <==
\begin{table*}[t]
    \centering 
    \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}p{0.05\linewidth}p{0.05\linewidth}p{0.42\linewidth}p{0.42\linewidth}@{}}
        \toprule 
        \textbf{Category} &\textbf{Reason} & \textbf{Question} & \textbf{Explanation} \\
        \toprule
        
        C1 & R1 &  What is minodixil approved for?& minodixil is a typo, the correct one is minoxidil\\
        \\
        C1 & R2 & List five proteins with antioxidant properties?  & BM25 fails to connect proteins and antioxidant properties, and retrieves documents all related to antioxidant, however, they are not about proteins nor antioxidant proteins.\\
        \\
        C1 & R2 & Has ZP-PTH been tested in a phase II clinical trial? & BM25 retrieves documents about phase II clinical trial but not about  ZP-PTH.\\
        \\
        C1 & R3 & How  large  is  a  lncRNAs? & BM25 retrieves document about lncRNAs but not about how large it is. \\
        \\
        C1 & R3 & Is indinavir effective for treatment of amyotrophic lateral sclerosis? & BM25 retrieves documents related to amyotrophic lateral sclerosis but not the treatments of amyotrophic lateral sclerosis. \\
        \\
        % C1 & R3 & What virus is the  Gardisil vaccine used for? &  BM25 retrieves documents about virus, but not Gardisil vaccine neither documents are about both of them.\\
        % \\
        C2 & R1 & What is Xanamem? & NR fails to retrieve any document related to Xanamem, rather, it retrieves documents that lexical similar to Xanamem such as Ximenia, Xadago, and Xenopus.\\
        \\
        C2 & R1 & What is Soluvia? & NR fails to retrieve any document related to Soluvia, rather, it retrieves documents that lexical similar to Soluvia such as Solexa, Saliva, and Viagra.\\
        \\
        C2 & R2 & Does an interferon (IFN) signature exist for SLE patients? & NR ranks documents about interferon higher than documents of SLE patients and documents of both. In the retrieved documents, interferon appears rather frequently. \\
        \bottomrule
    \end{tabular}
    }
    \caption{Examples of selected templates and generated questions for input texts based on template-based question generation approach.}
    \label{tab:error_analysis}
\end{table*}



==> index_units.tex <==
\begin{table}
    \centering
    % \small
    \resizebox{0.97\linewidth}{!}{
    \begin{tabular}{@{}cccllllll@{}}
    \toprule
    {\bf Index Unit} & {\bf Memory} & {\bf Time} &  {\bf B1}  & {\bf B2}  & {\bf B3}  & {\bf B4}  & {\bf B5} & {\bf Avg.}\\

    \toprule
    2-sents & 21G & RSM   &64.71& {\bf 64.92} &{\bf 64.28}  &{\bf 73.11}  & {\bf 66.29} &{\bf 66.66} \\
    128-chunk & 8.1G & RSM  &{\bf 65.16} & 63.24 &63.72  &72.13  & 65.29 & 65.91 \\
    256-chunk & 4.5G & RSM  & 63.76 & 59.71 &62.70 &67.21  & 64.17 & 63.51 \\
    512-abstract & 2.8G & RSM  & 61.92 & 57.84 &60.01 &61.11  & 62.66 & 60.71 \\
    \midrule
    2-sents & 21G & ETM  & {\bf 64.65} & \bf59.21 & 63.65  &\bf70.90 &\bf65.97 & \bf64.88  \\
    128-chunk & 8.1G & ETM  & 64.11 & 58.08 & \bf64.15  &69.90 & 63.16 & 63.88 \\
    256-chunk & 4.5G & ETM  &64.57 &58.51 & 64.02  &68.44 &62.6 & 63.62  \\
    512-abstract & 2.8G & ETM &60.06 &56.38 & 61.99  &65.01 &59.63 & 60.61 \\
    
    \toprule
    \end{tabular}
    }
    \caption{Two best NR models in short and long context: the first block is poly-DPR pretrained with RSM task and fine-tuned on TempQG(short); the second block is poly-DPR pretrained with ETM task and fine-tuned on TempQG(long). }
    \label{tab:inference_unit}
\end{table}

==> table_bio_examples.tex <==
\begin{table*}[t]
    \centering 
    \small
\resizebox{\linewidth}{!}{
    \begin{tabular}{@{}p{0.16\linewidth}p{0.26\linewidth}p{0.33\linewidth}p{0.19\linewidth}@{}}
        \toprule
        \textbf{Question} & \textbf{Answer} & \textbf{Retrieved Context (BM25)} & \textbf{Retrieved Context(DPR)} \\
        \toprule
    What is Soluvia? 
        & Soluvia by Becton Dickinson is a microinjection system for intradermal delivery of vaccines.
        & The US FDA approved Sanofi Pasteur's Fluzone Intradermal influenza vaccine that uses a new microinjection system for intradermal delivery of vaccines (Soluvia, Becton Dickinson).
        & Internet-ordered viagra (sildenafil citrate) is rarely genuine. \\
    \midrule
    Is BNN20 involved in Parkinson's disease?
        & BNN-20 could be proposed for treatment of PD
        & Rare causes of dystonia parkinsonism.
        & BNN-20 could be proposed for treatment of PD \\
    \midrule
    How large is a lncRNAs?
        & lncRNAs are defined as RNA transcripts longer than 200 nucleotides that are not transcribed into proteins.
        & lncRNAs are closely related with the occurrence and development of some diseases.
        & An increasing number of long noncoding RNAs (lncRNAs) have been identified recently. \\
    \bottomrule
    \end{tabular}
    }
    \caption{Illustrative example from the BioASQ challenge along with the context retrieved by two methods BM25~\cite{} and Dense Passage Retrieval~\cite{}. {\color{red} cite}}
    \label{tab:bio-example}
\end{table*}


==> table_main_result2.tex <==
\begin{table}
    \centering
    % \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}cccllllll@{}}
    \toprule
    {\bf Size} & {\bf PT} & {\bf FT} & {\bf B1}  & {\bf B2}  & {\bf B3}  & {\bf B4}  & {\bf B5} & {\bf Avg.}\\
    \toprule
    \multicolumn{3}{l}{\bf Small Corpus}\\
    \toprule
    128        & -        & BQ       &54.48      &50.51       &53.8       &59.06     &48.71     & 53.31 \\
    128        & RSM      & BQ       &65.94      &57.43       & 61.89     &69.01    &58.23      & 62.5  \\
    
    128 & -   & TempQG  &62.92  &58.79 &62.94 &70.3 &63.39 & 63.67  \\
    128 & RSM & TempQG  &{\bf 64.71} & {\bf 64.92} &{\bf 64.28}  &{\bf 73.11}  & {\bf 66.29} &{\bf 66.66} \\
    \midrule
    256 & - & BQ &35.69 &32.66  &32.26 &38.28  &30.87 & 33.95  \\
    256 & ICT & BQ &54.44  &47.37  &52.61 &53.69  &44.38 &50.50  \\
    256 & ETM & BQ &56.63 &46.63 &52.79 &56.97  &49.61 &52.53  \\
    256 & ICT+ETM & BQ &51.33 &49.43 &49.36 &53.19 &43.58 &49.38  \\
    256 & - & TempQG &63.95  & {\bf 59.51} &62.98 &66.71  &62.8 &63.19  \\
    256 & ETM & TempQG &64.57 &58.51 & {\bf 64.02}  &68.44 &62.6 & {\bf 63.62}  \\
    256 & ICT+ETM & TempQG & {\bf 64.93} &58.49  &60.18  &{\bf 69.42} & {\bf64.87} &63.58  \\
    \midrule
    BM25 & - & - &62.15  &61.3  &66.62  &74.14  &61.3  &65.10 \\
    \toprule
    \multicolumn{3}{l}{\bf Large Corpus}\\
    \toprule
    128 & RSM & TempQG & {\bf 35.1}  &29.07 &32.74 &33.31  &35.54 &33.15  \\
    BM25 & - & -  &28.5 &27.82  &37.97  &41.91  &35.42  &34.32 \\
    Hybrid & ~ & - &30.02 & {\bf 31.31} & {\bf 39.79} &{\bf 42.18}  & {\bf 37.99}  & {\bf 36.26} \\
    \toprule
    \end{tabular}
    }
    \caption{Performance of model trained by different techniques on BioASQ8 testing set, CS: context setting, PT: pretraining task, FT: finetuning task, Bi: batch i. BQ: BioASQ}
    \label{tab:main-result}
\end{table}

==> tempqg.tex <==
\begin{table*}[t]
    \centering 
    \small
\resizebox{0.85\linewidth}{!}{
    \begin{tabular}{@{}p{0.12\linewidth}p{0.8\linewidth}@{}}
        \toprule
        Input(C)
        & MiR-1 influences susceptibility to cardiac arrhythmias after myocardialinfarction.\\
   
        C $\rightarrow$ T 
        & is \_ influenced by \_ \\
        C, T $\rightarrow$ Q & Is  myocardial  infarctioninfluenced by MiR-1?\\
    \bottomrule
    \end{tabular}}
    \caption{Example how template-based questions are generated. The template extraction model retrieves possible templates (T), then question generator produces questions (Q). }
    \label{tab:tempqg}
\end{table*}

==> update_main_table.tex <==
\begin{table}
    \centering
    % \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}ccllllll@{}}
    \toprule
    {\bf PT} & {\bf FT} & {\bf B1}  & {\bf B2}  & {\bf B3}  & {\bf B4}  & {\bf B5} & {\bf Avg.}\\
    \toprule
    \multicolumn{3}{l}{\bf Small Corpus}\\
    \toprule
     -        & BQ(short)       &54.48      &50.51       &53.8       &59.06     &48.71     & 53.31 \\
    RSM      & BQ(short)       &65.94      &57.43       & 61.89     &69.01    &58.23      & 62.5  \\
    
    -   & TempQG(short)  &62.92  &58.79 &62.94 &70.3 &63.39 & 63.67  \\
    RSM & TempQG(short)  &{\bf 64.71} & {\bf 64.92} &{\bf 64.28}  &{\bf 73.11}  & {\bf 66.29} &{\bf 66.66} \\
    \midrule
    - & BQ(long) &35.69 &32.66  &32.26 &38.28  &30.87 & 33.95  \\
    ICT & BQ(long) &54.44  &47.37  &52.61 &53.69  &44.38 &50.50  \\
    ETM & BQ(long) &56.63 &46.63 &52.79 &56.97  &49.61 &52.53  \\
    ICT+ETM & BQ(long) &51.33 &49.43 &49.36 &53.19 &43.58 &49.38  \\
    - & TempQG(long) &63.95  & {\bf 59.51} &62.98 &66.71  &62.8 &63.19  \\
    ETM & TempQG(long) &64.57 &58.51 & {\bf 64.02}  &68.44 &62.6 & {\bf 63.62}  \\
    ICT+ETM & TempQG(long) & {\bf 64.93} &58.49  &60.18  &{\bf 69.42} & {\bf64.87} &63.58  \\
    \midrule
    BM25 & - &62.15  &61.3  &66.62  &74.14  &61.3  &65.10 \\
    Hybrid & - &66.30  &64.90  &69.54  &75.71  &64.82 &68.25 \\
    \toprule
    \multicolumn{3}{l}{\bf Large Corpus}\\
    \toprule
    RSM & TempQG(short) & {\bf 35.1}  &29.07 &32.74 &33.31  &35.54 &33.15  \\
    BM25 &  -  &28.5 &27.82  &37.97  &41.91  &35.42  &34.32 \\
    Hybrid & - &30.02 & {\bf 31.31} & {\bf 39.79} &{\bf 42.18}  & {\bf 37.99}  & {\bf 36.26} \\
    \toprule
    \end{tabular}
    }
    \caption{Performance of model trained by different techniques on BioASQ8 testing set, CS: context setting, PT: pretraining task, FT: finetuning task, Bi: batch i. BQ: BioASQ}
    \label{tab:update-main-result}
\end{table}
